Claim-Level Confidence Calibration for Reliable Decision Making with Large Language Models

Large Language Models (LLMs) increasingly support decision-making in high-stakes domains, but they often hallucinate and express confidence that is misaligned with factual correctness. Response-level confidence is a coarse signal: a single generation can mix correct and incorrect statements, so a single number is not actionable for users that must accept, reject, or verify individual pieces of information. We study claim-level confidence calibration as a decision-relevant uncertainty signal: each response is decomposed into atomic, verifiable claims, and each claim is assigned a calibrated confidence using inference-time signals from consistency across samples and self-verification. Our framework operates in closed-box settings (no logits, no fine-tuning) and applies post-hoc calibration directly at the claim level, enabling selective intervention such as evidence retrieval or human review for low-confidence claims. Across TriviaQA and TruthfulQA we evaluate seven baselines on six recent models (Llama-3.1, Mistral, Qwen2.5, DeepSeek-R1, GPT-4, GPT-4o), and show that claim-level decomposition combined with post-hoc calibration reduces expected calibration error on factual questions while exposing failure modes on adversarial false-premise questions where decision-makers most need reliable uncertainty estimates.

==> src/Fig_NIPS_tab/tab_summary_UQ.tex <==
\begin{table*}[!t]
    \caption{A summary of methods for uncertainty quantification(UQ) for classical deep learning. 
    % Upper side of the table lists the sampling-based UQ methods. \emph{``LLM scalable''} column indicates whether a UQ approach is computationally feasible or scalable to apply on large model architectures. {\xmark} indicates inapplicable, {\smark} indicates can be applied to certain layers. 
    }
    \centering
    \label{tab:base_methods_outline}
    \begin{tabular}{
    >{\arraybackslash}p{.2\textwidth}
    >{\arraybackslash}p{.24\textwidth}
    >{\arraybackslash}p{.24\textwidth} 
    >{\centering\arraybackslash}p{.15\textwidth}
    }
        \toprule
        \multicolumn{1}{c}{\textbf{Quantification Methods}}  & \multicolumn{1}{c}{\textbf{Advantages}}  & \multicolumn{1}{c}{\textbf{Limitations}} & \multirow{1}{*}{\textbf{LLM scalable}} \\ 
        \midrule

        BNN \cite{buntine1991bayesian, nix1994estimating, blundell2015bayesbybackprop, upadhyay2022bayescap} & Treat network weights as probability distributions for modeling the uncertainty. & Computational intensity of inference.  & \xmark \\
        Uncertainty-Aware training \cite{yan2023distortion} & Directly optimizes for uncertain samples. & Lack of works on designing effective loss functions and efficient integration. &  \smark \\
        Self-supervised learning \cite{kirchhof2023probabilistic} & Provides additional information about data distribution & Effectiveness depends on the chosen self-supervised task. & \smark \\
        
        \midrule

        Ensemble \cite{dietterich2000experimental} & Provides uncertainty through variability in predictions. & Can be computationally expensive. & \xmark  \\
        Deep Ensembles \cite{lakshminarayanan2017simple, dietterich2000experimental} & Better estimation with diversity. & Similar to regular ensembles, can be computationally expensive. & \xmark \\
        MCD \cite{gal2016dropout} & Captures uncertainty with Bayesian approximation. & Computationally expensive due to multiple forward passes. & \smark \\

        $O(N)$ Energy \cite{phasetransition2025} & Measure the intensity of interactions among tokens within the generated sentence. & Performs better on large models (>7B). & \smark \\

        \bottomrule
    \end{tabular}
\end{table*}

\eat{\begin{table*}[!t]
    \caption{A summary of methods for uncertainty quantification(UQ) for classical deep learning. The upper side of the table lists the sampling-based UQ methods. \emph{``LLM scalable''} column indicates whether a UQ approach is computationally feasible or scalable to apply on large model architectures. {\xmark} indicates inapplicable, {\smark} indicates can be applied to certain layers. }
    \centering
    \label{tab:base_methods_outline}
    \begin{tabular}{
    >{\arraybackslash}p{.2\textwidth}
    >{\arraybackslash}p{.24\textwidth}
    >{\arraybackslash}p{.24\textwidth} 
    >{\centering\arraybackslash}p{.1\textwidth}
    }
        \toprule
        \multicolumn{1}{c}{\textbf{Quantification Methods}}  &\multicolumn{1}{c}{\textbf{Advantages}}  & \multicolumn{1}{c}{\textbf{Limitations}}  & \multirow{1}{*}{\textbf{LLM scalable}} \\ 
        \midrule

        BNN \cite{buntine1991bayesian, nix1994estimating, blundell2015bayesbybackprop, upadhyay2022bayescap} & Treat network weights as probability distributions for modeling the uncertainty. & Computational intensity of inference.  & \xmark \\
        Uncertainty-Aware loss \cite{yan2023distortion} & Directly optimizes for uncertain samples. & Lack of works on designing effective loss functions and efficient integration. &  \smark \\
        Self-supervised learning \cite{kirchhof2023probabilistic} & Provides additional information about data distribution & Effectiveness depends on the chosen self-supervised task. & \smark \\
        
        \midrule

        Ensemble \cite{dietterich2000experimental} & Provides uncertainty through variability in predictions. & Can be computationally expensive. & \xmark  \\
        Deep Ensembles \cite{lakshminarayanan2017simple, dietterich2000experimental} & Better estimation with diversity. & Similar to regular ensembles, can be computationally expensive. & \xmark \\
        MCD \cite{gal2016dropout} & Captures uncertainty with Bayesian approximation. & Computationally expensive due to multiple forward passes. & \smark \\

        \bottomrule
    \end{tabular}
\end{table*}
}

==> src/Fig_NIPS_tab/tab_workshop_summary.tex <==
\begin{table*}[!htbp]
    \centering
    \caption{Condensed calibration results (ECE, smECE; lower is better)
      on TriviaQA and TruthfulQA across six models. We report a
      representative subset of baselines plus our verification-only
      instantiation ($\alpha{=}0$); best per model and dataset in bold. The
      full per-model table with BS, AUROC, BLEU, all baselines, and the
      tuned-$\alpha$ row is in Appendix~\ref{appendix:full_results}.}
    \label{tab:summary_results}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{ll|cc|cc}
    \toprule
    & & \multicolumn{2}{c|}{\textbf{TriviaQA}} & \multicolumn{2}{c}{\textbf{TruthfulQA}} \\
    \textbf{Model} & \textbf{Method} & ECE$\downarrow$ & smECE$\downarrow$ & ECE$\downarrow$ & smECE$\downarrow$ \\
    \midrule
    \multirow{4}{*}{\textbf{Llama-3.1-8B}}
      & Few-shot     & 0.046 & 0.040 & 0.386 & 0.333 \\
      & PS           & \bf 0.013 & \bf 0.013 & 0.363 & 0.319 \\
      & TS           & 0.045 & 0.039 & \bf 0.154 & \bf 0.154 \\
      & HalluMeasure & 0.242 & 0.127 & 0.989 & 0.394 \\
    \midrule
    \multirow{4}{*}{\textbf{Mistral-7B-v0.3}}
      & Few-shot     & 0.044 & 0.043 & 0.241 & 0.233 \\
      & PS           & \bf 0.010 & \bf 0.010 & 0.176 & 0.175 \\
      & TS           & 0.042 & 0.039 & \bf 0.057 & \bf 0.058 \\
      & HalluMeasure & 0.107 & 0.056 & 0.475 & 0.274 \\
    \midrule
    \multirow{4}{*}{\textbf{Qwen2.5-7B}}
      & Few-shot     & 0.310 & 0.286 & 0.187 & 0.185 \\
      & PS           & 0.142 & 0.141 & 0.363 & 0.320 \\
      & TS           & \bf 0.044 & \bf 0.037 & \bf 0.066 & \bf 0.067 \\
      & HalluMeasure & 0.242 & 0.121 & 0.983 & 0.403 \\
    \midrule
    \multirow{3}{*}{\textbf{GPT-4}}
      & Few-shot     & \bf 0.101 & \bf 0.075 & 0.325 & 0.232 \\
      & Verb.\ CoT   & 0.144 & 0.079 & 0.269 & 0.255 \\
      & TS           & 0.105 & 0.077 & \bf 0.230 & \bf 0.145 \\
    \midrule
    \multirow{5}{*}{\textbf{GPT-4o}}
      & Few-shot     & 0.090 & 0.079 & 0.277 & 0.259 \\
      & Few-shot CoT & \bf 0.027 & 0.034 & 0.488 & 0.345 \\
      & TS           & 0.096 & 0.085 & 0.118 & 0.116 \\
      & LMvsLM       & 0.171 & 0.087 & \bf 0.112 & \bf 0.097 \\
      & \cellcolor{yellow!50}\textbf{Ours} & \cellcolor{yellow!50}0.064 & \cellcolor{yellow!50}0.056 & \cellcolor{yellow!50}0.412 & \cellcolor{yellow!50}0.335 \\
    \midrule
    \multirow{5}{*}{\textbf{DeepSeek-R1}}
      & Verbalized      & 0.067 & 0.061 & 0.325 & 0.295 \\
      & Verbalized CoT  & 0.047 & 0.038 & 0.314 & 0.288 \\
      & LMvsLM          & 0.146 & 0.076 & \bf 0.066 & \bf 0.057 \\
      & HalluMeasure    & \bf 0.001 & \bf 0.001 & 0.584 & 0.379 \\
      & \cellcolor{yellow!50}\textbf{Ours} & \cellcolor{yellow!50}0.087 & \cellcolor{yellow!50}0.086 & \cellcolor{yellow!50}0.578 & \cellcolor{yellow!50}0.325 \\
    \bottomrule
    \end{tabular}}
\end{table*}

